Statistical Inference for Misspecified Contextual Bandits

Contextual bandit algorithms have transformed modern experimentation by enabling real-time adaptation for personalized treatment and efficient use of data. Yet these advantages create challenges for statistical inference due to adaptivity. A fundamental property that supports valid inference is policy convergence, meaning that action-selection probabilities converge in probability given the context. Convergence ensures replicability of adaptive experiments and stability of online algorithms. In this paper, we highlight a previously overlooked issue: widely used algorithms such as LinUCB may fail to converge when the reward model is misspecified, and such non-convergence creates fundamental obstacles for statistical inference. This issue is practically important, as misspecified models -- such as linear approximations of complex dynamic system -- are often employed in real-world adaptive experiments to balance bias and variance. Motivated by this insight, we propose and analyze a broad class of algorithms that are guaranteed to converge even under model misspecification. Building on this guarantee, we develop a general inference framework based on an inverse-probability-weighted Z-estimator (IPW-Z) and establish its asymptotic normality with a consistent variance estimator. Simulation studies confirm that the proposed method provides robust and data-efficient confidence intervals, and can outperform existing approaches that exist only in the special case of offline policy evaluation. Taken together, our results underscore the importance of designing adaptive algorithms with built-in convergence guarantees to enable stable experimentation and valid statistical inference in practice.

==> mystyle.tex <==
%-----------------------------------------------------------------%
%
% The latex macro
%
%-----------------------------------------------------------------%

\RequirePackage{amsmath}
\RequirePackage{amssymb}
\RequirePackage{amsthm}
\RequirePackage{bm}
\RequirePackage{url}
\usepackage{multirow}
%\usepackage{natbib}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{makecell}
\usepackage{booktabs}
\usepackage{array}
\usepackage{url}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{dsfont}
\usepackage{mathtools}
%\usepackage{xcolor}
\usepackage[title]{appendix}

% Comments
\usepackage{xcolor}
\newcount\comments  % 0 suppresses notes to selves in text
\comments=0  % TODO: change to 0 for final version
\newcommand{\genComment}[2]{\ifnum\comments=1{\textcolor{#1}{\textsf{\footnotesize #2}}}\fi}
\newcommand{\ambuj}[1]{\genComment{red}{[AT:#1]}}
\newcommand{\ziping}[1]{\genComment{green}{[ZP:#1]}}
\newcommand{\tarun}[1]{\genComment{blue}{[TG:#1]}}
\newcommand{\YG}[1]{\genComment{purple}{[YG:#1]}}

% -------- New Packages -------- %
\usepackage{enumitem}

%------ kpfonts -------%
%\usepackage{kpfonts}

%------- some other packages -------%
\usepackage{enumerate}
% \usepackage[OT1]{fontenc}
%\usepackage{natbib}
% \usepackage[usenames]{color}
%\usepackage[dvips]{graphicx}
%\usepackage[protrusion=true, expansion=true, tracking=true, spacing=true, final, babel]{microtype}
%\usepackage{makecell}
% \usepackage[colorlinks,
% linkcolor=blue,
% anchorcolor=blue,
% citecolor=blue
% ]{hyperref}
% \usepackage{hyperref}

%\usepackage{refcheck}

\usepackage{mathrsfs}
% \usepackage{fullpage}

%--------- new defs --------%



\def\TV{\mathop{\text{TV}}}
\def\supp{\mathop{\text{supp}}}
\def\card{\mathop{\text{card}}}
\def\rank{\mathrm{rank}}
\long\def\comment#1{}
\def\skeptic{{\sc skeptic}}
\def\NPN{\bPiox{\it NPN}}
\def\vec{\mathop{\text{vec}}}
\def\dr{\displaystyle \rm}
\def\OLS{\mathop{\text{OLS}}}
\def\ts{\textstyle}
\def\skeptic{{\sc skeptic}}
\providecommand{\bnorm}[1]{\Big\vvvert#1\Big\vvvert}
\providecommand{\norm}[1]{\vvvert#1\vvvert}
\def \txb {\overbar{\xb}}
\def \tx {\overbar{x}}

\def\bess{\bes\small }
\def\Shat{{\widehat S}}
\def\lam{\rho}
\def\real{{\mathbb{R}}}
\def\R{{\real}}
\def\Ti{T_{\rm init}}
\def\Tm{T_{\rm main}}
\def\bcdot{{\bm \cdot}}
\newcommand{\red}{\color{red}}
\newcommand{\blue}{\color{blue}}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\cIs}{\cI_{\hat{s}}}
\def \hbeta {\widehat{\beta}}

\let\oldemptyset\emptyset
\let\emptyset\varnothing


\newcommand{\dimq}{m_q}

\renewcommand{\baselinestretch}{1.1}

\def\sep{\;\big|\;}
\newcommand{\chz}[1]{{\textcolor{red}{[CHZ: #1]}}}
\newcommand{\hf}[1]{{\textcolor{red}{[FH: #1]}}}
\def \trunc{\mathop{\text{trunc}}}
\def \obs {{\rm obs}}
\def \mis {{\rm mis}}
\def \hbSigma {\widehat{\bSigma}}
\def \bbSigma {\bar{\bSigma}}


\newcommand{\tcT}{\tilde{\cT}}


%\usepackage[protrusion=false,expansion=true]{microtype}
%\usepackage[activate={true,nocompatibility},final,tracking=true,kerning=true,spacing=true,factor=1100,stretch=10,shrink=10]{microtype}


\def\##1\#{\begin{align}#1\end{align}}
\def\$#1\${\begin{align*}#1\end{align*}}

\let\cite\citet


\let\hat\widehat
\let\tilde\widetilde
\let\check\widecheck
\def\given{{\,|\,}}
\def\biggiven{{\,\big|\,}}
\def\Biggiven{{\,\Big|\,}}
\def\bigggiven{{\,\bigg|\,}}
\def\Bigggiven{{\,\Bigg|\,}}
\def\ds{\displaystyle}
\newcommand\wtilde{\stackrel{\sim}{\smash{\mathcal{W}}\rule{0pt}{1.1ex}}}



\newcommand{\eqal}[1]{\begin{equation}\begin{aligned} #1 \end{aligned}\end{equation}}
\newcommand{\bbr}[1]{\left[ {#1} \right]}
\newcommand{\bpa}[1]{\left( {#1} \right)}
\newcommand{\E}[1]{\textbf{E} \left[ {#1} \right]}
\newcommand{\pr}[1]{\textbf{P} \left({#1}\right)}
\newcommand{\nrm}[2]{\left \lVert {#2} \right \rVert_{#1}}


%----- bold fonts -----%

\newcommand{\ab}{\mathbf{a}}
\newcommand{\bbb}{\mathbf{b}}
\newcommand{\cbb}{\mathbf{c}}
\newcommand{\db}{\mathbf{d}}
\newcommand{\eb}{\mathbf{e}}
\newcommand{\fb}{\mathbf{f}}
\newcommand{\gb}{\mathbf{g}}
\newcommand{\hb}{\mathbf{h}}
\newcommand{\ib}{\mathbf{i}}
\newcommand{\jb}{\mathbf{j}}
\newcommand{\kb}{\mathbf{k}}
\newcommand{\lb}{\mathbf{l}}
\newcommand{\mb}{\mathbf{m}}
\newcommand{\nbb}{\mathbf{n}}
\newcommand{\ob}{\mathbf{o}}
\newcommand{\pb}{\mathbf{p}}
\newcommand{\qb}{\mathbf{q}}
\newcommand{\rb}{\mathbf{r}}
\newcommand{\sbb}{\mathbf{s}}
\newcommand{\tb}{\mathbf{t}}
\newcommand{\ub}{\mathbf{u}}
\newcommand{\vb}{\mathbf{v}}
\newcommand{\wb}{\mathbf{w}}
\newcommand{\xb}{\mathbf{x}}
\newcommand{\yb}{\mathbf{y}}
\newcommand{\zb}{\mathbf{z}}

\newcommand{\ba}{\bm{a}}
\newcommand{\bb}{\bm{b}}
\newcommand{\bc}{\bm{c}}
\newcommand{\bd}{\bm{d}}
\newcommand{\be}{\bm{e}}
\newcommand{\bbf}{\bm{f}}
\newcommand{\bg}{\bm{g}}
\newcommand{\bh}{\bm{h}}
\newcommand{\bi}{\bmf{i}}
\newcommand{\bj}{\bm{j}}
\newcommand{\bk}{\bm{k}}
\newcommand{\bl}{\bm{l}}
\newcommand{\bbm}{\bm{m}}
\newcommand{\bn}{\bm{n}}
\newcommand{\bo}{\bm{o}}
\newcommand{\bp}{\bm{p}}
\newcommand{\bq}{\bm{q}}
\newcommand{\br}{\bm{r}}
\newcommand{\bs}{\bm{s}}
\newcommand{\bt}{\bm{t}}
\newcommand{\bu}{\bm{u}}
\newcommand{\bv}{\bm{v}}
\newcommand{\bw}{\bm{w}}
\newcommand{\bx}{\bm{x}}
\newcommand{\by}{\bm{y}}
\newcommand{\bz}{\bm{z}}




\newcommand{\Ab}{\mathbf{A}}
\newcommand{\Bb}{\mathbf{B}}
\newcommand{\Cb}{\mathbf{C}}
\newcommand{\Db}{\mathbf{D}}
\newcommand{\Eb}{\mathbf{E}}
\newcommand{\Fb}{\mathbf{F}}
\newcommand{\Gb}{\mathbf{G}}
\newcommand{\Hb}{\mathbf{H}}
\newcommand{\Ib}{\mathbf{I}}
\newcommand{\Jb}{\mathbf{J}}
\newcommand{\Kb}{\mathbf{K}}
\newcommand{\Lb}{\mathbf{L}}
\newcommand{\Mb}{\mathbf{M}}
\newcommand{\Nb}{\mathbf{N}}
\newcommand{\Ob}{\mathbf{O}}
\newcommand{\Pb}{\mathbf{P}}
\newcommand{\Qb}{\mathbf{Q}}
\newcommand{\Rb}{\mathbf{R}}
\newcommand{\Sbb}{\mathbf{S}}
\newcommand{\Tb}{\mathbf{T}}
\newcommand{\Ub}{\mathbf{U}}
\newcommand{\Vb}{\mathbf{V}}
\newcommand{\Wb}{\mathbf{W}}
\newcommand{\Xb}{\mathbf{X}}
\newcommand{\Yb}{\mathbf{Y}}
\newcommand{\Zb}{\mathbf{Z}}

\newcommand{\bA}{\bm{A}}
\newcommand{\bB}{\bm{B}}
\newcommand{\bC}{\bm{C}}
\newcommand{\bD}{\bm{D}}
\newcommand{\bE}{\bm{E}}
\newcommand{\bF}{\bm{F}}
\newcommand{\bG}{\bm{G}}
\newcommand{\bH}{\bm{H}}
\newcommand{\bI}{\bm{I}}
\newcommand{\bJ}{\bm{J}}
\newcommand{\bK}{\bm{K}}
\newcommand{\bL}{\bm{L}}
\newcommand{\bM}{\bm{M}}
\newcommand{\bN}{\bm{N}}
\newcommand{\bO}{\bm{O}}
\newcommand{\bP}{\bm{P}}
\newcommand{\bQ}{\bm{Q}}
\newcommand{\bR}{\bm{R}}
\newcommand{\bS}{\bm{S}}
\newcommand{\bT}{\bm{T}}
\newcommand{\bU}{\bm{U}}
\newcommand{\bV}{\bm{V}}
\newcommand{\bW}{\bm{W}}
\newcommand{\bX}{\bm{X}}
\newcommand{\bY}{\bm{Y}}
\newcommand{\bZ}{\bm{Z}}


%----- calligraphic fonts -----%

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{{\mathcal{S}}}
\newcommand{\cT}{{\mathcal{T}}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}


\newcommand{\sB}{\mathscr{B}}



%----- blackboard bold fonts-----%

\newcommand{\BB}{\mathbb{B}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\VV}{\mathbb{V}}
\newcommand{\II}{\mathbb{I}}
\newcommand{\KK}{\mathbb{K}}
\newcommand{\LL}{\mathbb{L}}
\newcommand{\MM}{\mathbb{M}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\SSS}{\mathbb{S}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\OOmega}{\mathbb{\Omega}}




%----- bold greek fonts -----%

\newcommand{\balpha}{\bm{\alpha}}
\newcommand{\bbeta}{\bm{\beta}}
\newcommand{\bgamma}{\bm{\gamma}}
\newcommand{\bepsilon}{\bm{\epsilon}}
\newcommand{\bvarepsilon}{\bm{\varepsilon}}
\newcommand{\bzeta}{\bm{\zeta}}
\newcommand{\btheta}{\bm{\theta}}
\newcommand{\bvartheta}{\bm{\vartheta}}
\newcommand{\bkappa}{\bm{\kappa}}
\newcommand{\blambda}{\bm{\lambda}}
\newcommand{\bmu}{\bm{\mu}}
\newcommand{\bnu}{\bm{\nu}}
\newcommand{\bxi}{\bm{\xi}}
\newcommand{\bpi}{\bm{\pi}}
\newcommand{\bvarpi}{\bm{\varpi}}
\newcommand{\brho}{\bm{\varrho}}
\newcommand{\bsigma}{\bm{\sigma}}
\newcommand{\bvarsigma}{\bm{\varsigma}}
\newcommand{\btau}{\bm{\tau}}
\newcommand{\bupsilon}{\bm{\upsilon}}
\newcommand{\bphi}{\bm{\phi}}
\newcommand{\bvarphi}{\bm{\varphi}}
\newcommand{\bchi}{\bm{\chi}}
\newcommand{\bpsi}{\bm{\psi}}
\newcommand{\bomega}{\bm{\omega}}

\newcommand{\bGamma}{\bm{\Gamma}}
\newcommand{\bDelta}{\bm{\Delta}}
\newcommand{\bTheta}{\bm{\Theta}}
\newcommand{\bLambda}{\bm{\Lambda}}
\newcommand{\bXi}{\bm{\Xi}}
\newcommand{\bPi}{\bm{\Pi}}
\newcommand{\bSigma}{\bm{\Sigma}}
\newcommand{\bUpsilon}{\bm{\Upsilon}}
\newcommand{\bPhi}{\bm{\Phi}}
\newcommand{\bPsi}{\bm{\Psi}}
\newcommand{\bOmega}{\bm{\Omega}}


%----- Some standard definitions -----%

\newcommand{\independent}{\perp\!\!\!\!\perp}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand{\arginf} {\mathop{\mathrm{arginf}}}
\newcommand{\minimize}{\mathop{\mathrm{minimize}}}

\newcommand{\sign}{\mathop{\mathrm{sign}}}
\newcommand{\tr}{\mathop{\mathrm{tr}}}
\newcommand{\trace}{\mathop{\mathrm{Trace}}}

\DeclareMathOperator{\Var}{{\rm Var}}
\DeclareMathOperator{\Cor}{\rm Corr}
\DeclareMathOperator{\Cov}{\rm Cov}
\DeclareMathOperator{\ind}{\mathds{1}}  % Indicator
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}

\newcommand*{\zero}{{\bm 0}}
\newcommand*{\one}{{\bm 1}}

\newcommand{\diag}{{\rm diag}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%% Norms
\newcommand{\fro}{\mathop{\mathrm{fro}}}
\newcommand{\oper}{\mathop{\mathrm{op}}}

%%%%% Dot product
\newcommand{\dotp}[2]{\langle{#1},{#2}\rangle}

%%%%  brackets
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abr}[1]{\left|#1\right|}

%%%%%%%%%  Other commands

\newcommand{\mcomment}[1]{\marginpar{\tiny{#1}}}
\newcommand{\fcomment}[1]{\footnote{\tiny{#1}}}
\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}
\newcommand{\ud}{{\mathrm{d}}}


%%%%%%%%  amsmath %%%%%%%%%%
\newtheoremstyle{mytheoremstyle} % name
    {\topsep}                    % Space above
    {\topsep}                    % Space below
    {\normalfont}                   % Body font
    {}                           % Indent amount
    {\bfseries}                   % Theorem head font
    {.}                          % Punctuation after theorem head
    {.5em}                       % Space after theorem head
    {}  % Theorem head spec (can be left empty, meaning ‘normal’)

% \theoremstyle{mytheoremstyle}

% \ifx\BlackBox\undefined
% \newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % end of proof
% \fi

% \ifx\QED\undefined
% \def\QED{~\rule[-1pt]{5pt}{5pt}\par\medskip}
% \fi

% \ifx\proof\undefined
% \newenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox\\[2mm]}
% %\newenvironment{proof}{\emph{Proof. }}{ \hfill \QED}
% \fi

% \ifx\theorem\undefined
% \newtheorem{theorem}{Theorem}[section]
% \fi
% \ifx\example\undefined
% %\newtheorem{example}[theorem]{Example}
% %\newtheorem{example}{Example}[section]
% \fi
% \ifx\property\undefined
% \newtheorem{property}{Property}[section]
% \fi
% \ifx\lemma\undefined
% %\newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{lemma}{Lemma}[section]
% \fi
% \ifx\proposition\undefined
% %\newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{proposition}{Proposition}[section]
% \fi
% \ifx\remark\undefined
% %\newtheorem{remark}[theorem]{Remark}
% \newtheorem{remark}{Remark}[section]
% \fi
% \ifx\corollary\undefined
% %\newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{corollary}{Corollary}[section]
% \fi
% \ifx\definition\undefined
% %\newtheorem{definition}[theorem]{Definition}
% \newtheorem{definition}{Definition}[section]
% \fi
% \ifx\conjecture\undefined
% %\newtheorem{conjecture}[theorem]{Conjecture}
% \newtheorem{conjecture}{Conjecture}[section]
% \fi
% \ifx\fact\undefined
% %\newtheorem{fact}[theorem]{Fact}
% \newtheorem{fact}{Fact}[section]
% \fi
% \ifx\claim\undefined
% %\newtheorem{claim}[theorem]{Claim}
% \newtheorem{claim}{Claim}[section]
% \fi
% \ifx\assumption\undefined
% %\newtheorem{assumption}[theorem]{Assumption}
% \newtheorem{assumption}{Assumption}[section]
% \fi
% \ifx\cond\undefined
% %\newtheorem{cond}[theorem]{Condition}
% \newtheorem{cond}{Condition}[section]
% \fi

% \newtheoremstyle{anothertheoremstyle} % name
%     {\topsep}                    % Space above
%     {\topsep}                    % Space below
%     {\normalfont}                   % Body font
%     {}                           % Indent amount
%     {\bfseries}                   % Theorem head font
%     {.}                          % Punctuation after theorem head
%     {.5em}                       % Space after theorem head
%     {\thmname{#1} \thmnumber{#2} \normalfont{#3}}  % Theorem head spec (can be left empty, meaning ‘normal’)
% \ifx\condition\undefined
% \theoremstyle{anothertheoremstyle}
% %\newtheorem{condition}[theorem]{Condition}
% \newtheorem{condition}{Condition}
% \fi
% \numberwithin{equation}{section}
% \numberwithin{theorem}{section}

% \makeatletter
% \newcommand{\raisemath}[1]{\mathpalette{\raisem@th{#1}}}
% \newcommand{\raisem@th}[3]{\raisebox{#1}{$#2#3$}}
% \makeatother

% \let\oldabstract\abstract
% \let\oldendabstract\endabstract
% \makeatletter
% \renewenvironment{abstract}
% {\renewenvironment{quotation}%
%                {\list{}{\addtolength{\leftmargin}{-0.5em} % change this value to add or remove length to the the default
%                        \listparindent 0em%
%                         \itemindent    \listparindent%
%                         \rightmargin   \leftmargin%
%                         \parsep        \z@ \@plus\p@}%
%                 \item\relax}%
%                {\endlist}%
% \oldabstract}
% {\oldendabstract}
% \makeatother

